Applying Wirtinger derivatives to the radio interferometry calibration problem

This paper presents a fast algorithm for full-polarisation, direction dependent calibration in radio interferometry. It is based on Wirtinger's approach to complex differentiation. Compared to the classical case, and under reasonable approximations, the Jacobian appearing in the Levenberg-Maquardt iterative scheme presents a sparse structure, allowing for high gain in terms of algorithmic cost.

==> Connection.tex <==
\section{Connection with other existing algorithms}
\label{sec:Connection}

In this section, we investigate the connections between the complex
optimisation point of view (see Sec. \ref{sec:Wirtinger} and
\ref{sec:Solver}) and the existing algorithm. We show that antenna
based calibration schemes are always obtainable using this framework,
while general pealing based approaches are appliable under certain condition
of orthogonality between Fourier kernels.


\subsection{Levenberg-Maquardt and pealing}

\subsection{\sc{StefCal}}



